ProbTA: A sound and complete proof rule for probabilistic verification

We propose a sound and complete proof rule ProbTA for quantitative analysis of violation probability of probabilistic programs. Our approach extends the technique of trace abstraction with probability in the control-flow randomness style, in contrast to previous work of combining trace abstraction and probabilisitic verification which adopts the data randomness style. In our method, a program specification is proved or disproved by decomposing the program into different modules of traces. Precise quantitative analysis is enabled by novel models proposed to bridge program verification and probability theory. Based on the proof rule, we propose a new automated algorithm via CEGAR involving multiple technical issues unprecedented in non-probabilistic trace abstraction and data randomness-based approach.

==> experiment.tex <==
% !TEX root = ./main.tex

\paragraph{Implementation} To further illustrate the effectiveness of our framework, we implement the automated verification algorithm in a prototype tool written in Java. We use \textsc{SMTInterpol}\cite{smt_interpol}, an SMT solver with interpolation support, as the underlying solver. Essentially there is no restriction (except for the deterministic requirement) for expression and variable type in our framework. The implementation, however, only supports boolean and integer types and expressions in linear integer arithmetics, due to the limitation of state-of-the-art interpolation solvers.

\paragraph{Benchmarks} We evaluate our algorithm on two sets of benchmarks. 

\begin{itemize}
    \item \textsc{Violation:} We collected 9 examples from Wang et al.~\cite{exponential_analysis_of_probabilistic_program}, a recent work that implements algorithms to compute upper and lower bounds of assertion violation probability of probabilistic program. We altered these examples and used our algorithm to verify the violation bounds computed by \cite{exponential_analysis_of_probabilistic_program}. These examples, however, are too large-scale with counterexamples consisting of up to 1,000,000,000 traces. We then instead test the same examples with smaller scale, where our algorithm even obtained the exact violation probability.
    \item \textsc{Crafted:} This category contains a total of 16 programs adapted from  problem of interests in the probabilistic verification and termination analysis literature\cite{termination_positivstellensatz,mciver2005abstraction} and classical probability theory.
\end{itemize}

%\tbd{
%The examples we tested are mainly from several related works with some modification, 
%details of which, in the interests of space, are documented in \cref{sec: testsuit}.
%\todo{Guanyan modified}
%}

\paragraph{Results} Our experimental results are summarised in \cref{table: result}. For SAT cases we give the upper bound of violation probability computed by our algorithm, while for UnSAT cases, we give the number of traces in the counterexample and the overall violation probability of the counterexample\footnote{In this case our algorithm also returns a precondition under which the counterexample is enabled. It could, however, get very complicated and is thus omitted. }. The number of CEGAR iterations needed to prove or disprove the property is also given.

\begin{table*}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|} 
        \hline
\multicolumn{2}{|c|}{\textbf{Benchmark}}                                                                 & $\bm{\beta}$ & \textbf{Result} & \textbf{\#Iteration} & \begin{tabular}[c]{@{}c@{}}\textbf{Upper Bound}\\\textbf{of V.P.}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\#Traces}\\\textbf{in Counterexample}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Overall V.P. of }\\\textbf{Counterexample}\end{tabular}  \\ 
\hline
\hline
\multirow{8}{*}{\rotatebox[origin=c]{90}{\textsc{Violation}}} & \textsc{1DWalk}                                                            & $1 \times 10^{-6}$ & UnSAT       & 13                   & -                                                                              & 1                                                                                     & $2.4414\times 10^{-4}$                                                                      \\ 
\cline{2-8}
                                     & \textsc{2DWalk}                                                            & 0.2                & SAT         & 4                    & 0.1852                                                                         & -                                                                                     & -                                                                                           \\ 
\cline{2-8}
                                     & \textsc{3DWalk}                                                            & 0.01               & SAT         & 19                   & 0.001193                                                                       & -                                                                                     & -                                                                                           \\ 
\cline{2-8}
                                     & \textsc{Coupon5}                                                           & 0.2                & UnSAT       & 9                    & -                                                                              & 41                                                                                    & 0.2004                                                                                      \\ 
\cline{2-8}
                                     & \textsc{Prspeed}                                                           & 0.01               & UnSAT       & 25                   & -                                                                              & 481                                                                                   & 0.010009                                                                                    \\ 
\cline{2-8}
                                     & \textsc{Race}                                                              & 0.03125            & SAT         & 6                    & 0.03125                                                                        & -                                                                                     & -                                                                                           \\ 
\cline{2-8}
                                     & \textsc{RdAdder}                                                           & 0.08               & SAT         & 110                  & 0.0796                                                                         & -                                                                                     & -                                                                                           \\ 
\cline{2-8}
                                     & \textsc{RdWalk}                                                            & 0.01               & UnSAT       & 9                    & -                                                                              & 1                                                                                     & 0.0751                                                                                      \\ 
\hline
\multirow{15}{*}{\rotatebox[origin=c]{90}{\textsc{Crafted}}}  & \textsc{GamblerRuin}                                                       & 0.75               & UnSAT       & 2                    & -                                                                              & 16                                                                                    & 0.7504                                                                                      \\ 
\cline{2-8}
                                     & \textsc{GamblerEquiv}                                                      & 0.01               & SAT         & 2                    & 0.0                                                                            & -                                                                                     & -                                                                                           \\ 
\cline{2-8}
                                     & \textsc{Coupon3}                                                           & 0.04                & SAT         & 23                    & 0.03840                                                                          & -                                                                                     & -                                                                                           \\ 
\cline{2-8}
                                     & \textsc{Herman2}                                                           & 0.1                & UnSAT       & 9                    & -                                                                              & 1                                                                                     & 0.125                                                                                       \\ 
\cline{2-8}
                                     & \textsc{Limit} & 0.3               & UnSAT       & 3                    & -                                                                              & 3                                                                                    & 0.375                                                                                      \\ 
\cline{2-8}
                                     & \textsc{LimitV}                                                            & 0.47               & UnSAT       & 4                    & -                                                                              & 31                                                                                    & 0.4843                                                                                      \\ 
\cline{2-8}
                                     & \textsc{LimitV2}                                                           & 0.47               & SAT         & 6                    & 0.4433                                                                         & -                                                                                     & -                                                                                           \\ 
\cline{2-8}
                                     & \textsc{MultiProb}                                                         & 0.85               & SAT         & 4                    & 0.85000                                                                        & -                                                                                     & -                                                                                           \\ 
\cline{2-8}
                                     & \textsc{NonProb}                                                           & 0.0                & SAT         & 2                    & 0.0                                                                            & -                                                                                     & -                                                                                           \\ 
\cline{2-8}
                                     & \textsc{RandomWalk}                                                        & 0.95               & UnSAT       & 2                    & -                                                                              & 82                                                                                    & 0.95001                                                                                     \\ 
\cline{2-8}
                                     & \textsc{Sample}                                                            & 0.04               & UnSAT       & 6                    & -                                                                              & 32                                                                                     & 0.040039                                                                                    \\ 
\cline{2-8}
                                     & \textsc{Sum}                                                               & 0.1                & UnSAT       & 3                    & -                                                                              & 1                                                                                     & 0.125                                                                                       \\ 
\cline{2-8}
                                     & \textsc{ThreeDoor}                                                         & 0.34               & SAT         & 12                   & 0.33                                                                           & -                                                                                     & -                                                                                           \\ 
\cline{2-8}
                                     & \textsc{ThreeUp}                                                           & 0.33               & UnSAT       & 2                    & -                                                                              & 2                                                                                     & 0.4389                                                                                      \\ 
\cline{2-8}
                                     & \textsc{Uniform}                                                           & 0.334              & SAT         & 4                    & 0.333                                                                          & -                                                                                     & -                                                                                           \\
                                     \hline
\end{tabular}
    \bigskip
    \caption{Experimental Results for our algorithm, where V.P. stands for violation probability, SAT means the actual violation probability is below the expected one, $\beta$ is the expected violation probability, and \#Iteration is the total number of CEGAR iterations taken during the algorithm.}
    \label{table: result}
\end{table*}

\paragraph{Discussion}
The experimental results show the effectiveness of our verification algorithm. The bound of violation probability of most cases could be obtained in a small number of iterations. The bound computed is close to the actual violation probability and, in certain cases (like \textsc{Race}), a precise bound could be computed. On the other hand, the case \textsc{RdAdder} needs 110 iterations to find the proof, mainly because of the large scale of the trace sets. However, 109 out of these iterations are dealing with non-violating traces, corrsponding to the right loop in \cref{figure: algorithm framework}. Essentially, our algorithm use non-violating generalization (without considering probability) to shrink down the trace set as much as possible.
